Semi-Supervised Domain Generalization for Object Detection via Language-Guided Feature Alignment

Existing domain adaptation (DA) and generalization (DG) methods in object detection enforce feature alignment in the visual space but face challenges like object appearance variability and scene complexity, which make it difficult to distinguish between objects and achieve accurate detection. In this paper, we are the first to address the problem of semi-supervised domain generalization by exploring vision-language pre-training and enforcing feature alignment through the language space. We employ a novel Cross-Domain Descriptive Multi-Scale Learning (CDDMSL) aiming to maximize the agreement between descriptions of an image presented with different domain-specific characteristics in the embedding space. CDDMSL significantly outperforms existing methods, achieving 11.7% and 7.5% improvement in DG and DA settings, respectively. Comprehensive analysis and ablation studies confirm the effectiveness of our method, positioning CDDMSL as a promising approach for domain generalization in object detection tasks.

==> Experiments.tex <==
\section{Experiments}
\label{sec:experiments} %added after deadline
\textbf{Real-to-artistic generalization.} We conduct our experiments based on 4 %publicly available 
datasets:  Pascal-VOC (VOC) \cite{pascal-voc-2012,pascal-voc-2007}, Clipart1k \cite{inoue2018cross}, Watercolor2k \cite{inoue2018cross}, Comic2k \cite{inoue2018cross} to assess generalizability on artistic and style domain shifts. VOC contains 20 categories of common objects from 16,551 natural images, Clipart consists of 20 categories of 3,165 objects from 1000 instances, and Watercolor and Comic contain 6 categories of 3,315 and 6,389 objects from 2,000 images, respectively. Experiments are conducted in three settings: (1) VOC and Clipart, (2) VOC and Watercolor, and (3) VOC and Comic are used as the source domains, in which only VOC is considered a labeled domain. In each setting, the remaining datasets are considered as unseen targets %in the inference 
to assess the generalizability of the model across multiple domains (Table \ref{tab:DG-voc}). We further extend our model to DA and show the results in the supplement.

\textbf{Adverse weather adaptation.} %Similar to DIDN, 
We experiment on Cityscapes \cite{Cordts2016Cityscapes} (City), Foggy-Cityscapes \cite{Cordts2016Cityscapes} (Foggy), and BDD100k \cite{bdd100k} (Bdd) to evaluate generalizability across different time and weather conditions. City features 3,025 urban images from 50 cities, while Foggy simulates fog on City, and Bdd comprises 10,000 images of various weather conditions and times. All datasets contain 8 categories, but we ignore the ``train'' category on Bdd due to its low instance count on the validation set \cite{lin2021domain}. As Foggy is a simulated based on City, we use them as the source domains without the need for style transfer (City labeled and Foggy unlabeled), while Bdd is an unseen target (results in supplement). Note we do not use the labels on the Foggy data throughout training. Following DIDN \cite{lin2021domain}, since most of the previous works are on weather adaptation, we perform adaptation from City to Foggy and extensively compare against baselines and related works as shown in Table \ref{tab:uda-c2fc}.

\textbf{Baselines.}
\label{sec:baselines}
Faster-RCNN \cite{ren2015faster} (F-RCNN) with ImageNet \cite{deng2009imagenet} and RegionCLIP (R-CLIP) are labeled source-only baselines, trained on VOC for real-to-artistic generalization (Table \ref{tab:DG-voc}, \ref{tab:ablation_all}) and City for adverse weather adaptation (Table \ref{tab:uda-c2fc}). For a fair comparison, we only compare against models using ResNet50 backbone as RegionCLIP \cite{zhong2022regionclip} does not have ResNet101 pre-trained weights available. For real-to-artistic generalization, we further train Adaptive-MT
% \footnote{\url{https://yujheli.github.io/projects/adaptiveteacher.html}} 
\cite{li2022cross}, a state-of-the-art (sota) DA with ResNet50 backbone. We define \textit{Direct Visual Alignment} (DVA) and \textit{Caption Pseudo Labeling} (Caption-PL) as additional baselines in the ablation (see Table \ref{tab:ablation_all}). DVA applies the descriptive consistency loss in the visual space without using $v2l$. Caption-PL uses pseudo labels obtained by applying ClipCap on the original image to compute image-captioning loss over tokens for the stylized image. IRG \cite{vs2022instance} is only reported for the (VOC and Clipart) setting 
%to maintain a fair comparison, 
as performance/pretrained weights were reported only in this setting. See supplement for more discussion of our choice of baselines.

\textbf{Implementation details.} PyTorch \cite{NEURIPS2019_9015} and Detectron2 \cite{wu2019detectron2} are used for development. RegionCLIP's ResNet50 \cite{he2016deep} is adopted as the object detector backbone. Following ClipCAP\footnote{\url{https://github.com/rmokady/CLIP_prefix_caption}}, $v2l$ consists of 8 multi-head self-attention layers with
8 heads, pre-trained along with RegionCLIP encoder and GPT-2 on COCO-captions \cite{chen2015microsoft,lin2014microsoft}, in which RegionCLIP stays frozen. Projection layer $g$ (after $\textit{v2l}$ in Fig.\ref{fig:model}) has  output dimension 256. SGD with an initial lr of 0.002, linear scheduler, and a batch size of 8 is used for all experiments except the RegionCLIP baseline, which uses a batch size of 12. Experiments are conducted on 4 NVIDIA Quadro RTX 5000 with 10k burn-up and 20k joint-training iterations. The burn-up stage is performed following RegionCLIP, and SSDG experiments continue from this checkpoint. $\omega$ is set to 1 in $\mathcal{L}_{tot}$. We evaluate mAP with a
threshold of 0.5.
% with results chosen based on the best validation score using the unlabeled source domain as the validation set.
\subsection{Results}

\begin{table}[!tp]
\scriptsize
\centering
  \captionsetup{skip=0pt, position=above} % Force the caption to be above the table
 \caption{\textbf{Real-to-artistic generalizations}. Numbers in parentheses show the difference from RegionCLIP. Max $\uparrow$ shows maximum improvement over two target domains compared to F-RCNN. We report mAP ($\%$). $\dagger$/$\ddagger$ denote DA methods/labeled source-only methods.
 %, respectively.
 }
  \label{tab:DG-voc}
\begin{tabular}{@{\hspace{3pt}}llllllll@{\hspace{1pt}}} 
\toprule
% \grayrow
    \multirow{2}{*}{{Method}}&
    \multicolumn{2}{l}{{VOC\&Clip \textrightarrow Water,Com}}  & 
    \multicolumn{2}{l}{{VOC\&Water\textrightarrow Clip,Com}} &
    \multicolumn{2}{l}{{VOC\&Com\textrightarrow Clip,Water}}&
    \multirow{2}{*}{Max $\uparrow$ }\\  
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule{6-7}
& Watercolor&Comic&Clipart&Comic&Clipart&Watercolor&\\
\hline
\multicolumn{1}{l|}{F-RCNN$\ddagger$ \cite{ren2015faster}} &41.2&17.9&24.1&17.9&24.1&41.2&\multicolumn{1}{|l}{-}\\
\multicolumn{1}{l|}{R-CLIP$\ddagger$ \cite{zhong2022regionclip}}  &44.7&34.2&33.9&34.2&33.9&44.7&\multicolumn{1}{|@{\hspace{3pt}}l@{\hspace{3pt}}}{16.3/16.3/9.8}\\
\hline
\multicolumn{1}{l|}{Adaptive MT$\dagger$ \cite{li2022cross}} &40.6 \tiny{\textcolor{red}{(-4.1)}}&22.2 \tiny{\textcolor{red}{(-12.0)}}&29.0 \tiny{\textcolor{red}{(-4.9)}}&24.3 \tiny{\textcolor{red}{(-9.9)}}&25.7 \tiny{\textcolor{red}{(-8.2)}}&42.3 \tiny{\textcolor{red}{(-2.4)}}&\multicolumn{1}{|@{\hspace{3pt}}l@{\hspace{0pt}}}{4.3/6.4/1.6}\\
\multicolumn{1}{l|}{IRG$\dagger$ \cite{vs2022instance}} &48.1 \tiny{\textcolor{blue}{(+3.4)}}&25.9 \tiny{\textcolor{red}{(-8.3)}}&-&-&-&-&\multicolumn{1}{|@{\hspace{3pt}}l@{\hspace{3pt}}}{8.0/-/-}\\
\multicolumn{1}{l|}{\textbf{Ours}}  &\textbf{49.8} \tiny{\textcolor{blue}{(+5.1)}}&\textbf{45.9} \tiny{\textcolor{blue}{(+11.7)}}&\textbf{38.7} \tiny{\textcolor{blue}{(+4.8)}}&\textbf{43.5} \tiny{\textcolor{blue}{(+9.3)}}&\textbf{39.8} \tiny{\textcolor{blue}{(+5.9)}}&\textbf{49.4} \tiny{\textcolor{blue}{(+5.2)}}&\multicolumn{1}{|@{\hspace{3pt}}l@{\hspace{3pt}}}{\textbf{28.0}/\textbf{25.6}/\textbf{15.7}}\\
% Target only & && & &\\
\bottomrule
\end{tabular}
\end{table}

\textbf{Vision-language pre-training.} According to  Table \ref{tab:DG-voc}, RegionCLIP solely significantly improves the generalizability of Faster-RCNN by $9.8\%$, $3.5\%$, and $16.3\%$ on Clipart, Watercolor, and Comic respectively. Additionally, we observe $6.5\%$ improvement on \textit{City,Foggy $\rightarrow$ Bdd} (in supplement). These results support our first observation, the advantage of vision-language pre-training (Sec.~\ref{sec:intro}). Table \ref{tab:uda-c2fc} demonstrates the efficacy of vision-language pertaining to DA as well (compare rows 1 and 2). We further improve RegionCLIP initialization by incorporating descriptive consistency learning as described in section \ref{sec:CDDMSL}.

\textbf{Domain generalization results.} 
 Table \ref{tab:DG-voc} showcases the generalizability of our proposed method on real-to-artistic tasks. The table is divided into three sections according to the unlabeled domain (i.e., Clipart, Watercolor, and Comic). Our proposed method consistently enhances RegionCLIP generalizability by and achieves the best result compared to the DA baselines by a large margin. For example, it achieves an $11.7\%$ and $9.3\%$ improvement on Comic when Clipart and Watercolor is the unlabeled source, respectively. We also observe that baselines perform better on Watercolor, which is intuitive as Watercolor is the closest domain to VOC. Likewise, our proposed approach outperforms DIDN on \textit{City,Foggy $\rightarrow$ Bdd} by $4.45\%$ (see supplement). These results demonstrate the effectiveness of language-guided feature alignment and the proposed consistency learning method for developing a generalized object detector. 
 
 % against traditional methods in object detection. 
% \begin{table}[!tp]\centering
% \scriptsize
% \captionsetup{skip=0pt, position=above} % Force the caption to be above the table
% \caption{\textbf{Domain adaptation.} City\textrightarrow Foggy in mAP ($\%$), $\dagger$ is source-free DA.}
% \label{tab:uda-c2fc}
% \begin{tabular}{l|@{\hspace{3pt}}l@{\hspace{2pt}}|cccccccc|l}
% \hline
%  &\textbf{Method}  &\textbf{prsn} &\textbf{rider} &\textbf{car} &\textbf{truck} &\textbf{bus} &\textbf{train} &\textbf{motor} 
% &\textbf{bike} & \textbf{mAP} \\
% \hline
% \multirow{2}{*}{-}&F-RCNN \cite{ren2015faster}& 26.9 & 38.2 & 35.6& 18.3& 32.4&9.6 & 25.8& 28.6&26.9\textcolor{red}{\tiny{(-22.1)}} \\
% &R-CLIP \cite{zhong2022regionclip} &46.5 &51.8 &57.6 &27.3 &45.1 & 19.7& 34.8& 50.2 &41.6\textcolor{red}{\tiny{(-7.5)}} \\
% \hline
%  \multirow{9}{*}{DA}&SW-DA \cite{saito2019strong}\tiny(CVPR'19) &31.8 & 44.3&48.9 &21.0 &43.8 &28.0&28.9 &35.8& 35.3\\
%  &MTOR \cite{cai2019exploring} \tiny(CVPR'19)  &30.6 &41.4 &44.0 &21.9  &38.6 &40.6 &28.3 &35.6 & 35.1\\
%  &ICR-CCR \cite{xu2020exploring} \tiny(CVPR'20) &32.9 &43.8 &49.2 &27.2 &45.1 &36.4 &30.3 &34.6 & 37.4\\
%  &Coarse-to-Fine \cite{zheng2020cross} \tiny(CVPR'20)  & 34.0& 46.9& 52.1& 30.8& 43.2& 29.9& 34.7& 37.4& 38.6\\
%  &GPA \cite{xu2020cross} \tiny(CVPR'20)  & 32.9&46.7 &54.1 &24.7 &45.7 &41.1 &32.4 &38.7 & 39.5\\ 
%  &Center-Aware \cite{hsu2020every} \tiny(ECCV'20)  &41.5 &43.6 &57.1 &29.4 &44.9 &39.7 &29.0 &36.1 & 40.2\\ 
%  &CycConf \cite{wang2021robust}\tiny(ICCV'21)  &45.8 &51.0 &63.1 &26.8 &47.1 &23.6 & 30.6& 43.6&41.5 \\
%  &TTD+FPN \cite{he2022cross} \tiny(CVPR'22) & 50.7 & 53.7 & 68.2 & 35.1 & 53.0 & 45.1 & 38.9 &49.1 & \textbf{49.2}\\
%  &IRG $\dagger$\tablefootnote{Source-free domain adaptation} \cite{vs2022instance} \tiny(CVPR'23)  & 37.4& 45.2& 51.9& 24.4& 39.6& 25.2& 31.5 &41.6 &  37.1\\
%  \hline
%  \multirow{2}{*}{DG}&DIDN \cite{lin2021domain} \tiny(ICCV'21)  &38.3 &44.4 &51.8 &28.7 &53.3 &34.7 &32.4 & 40.4&40.5\textcolor{red}{\tiny{(-8.6)}} \\
% &\textbf{Ours}  &50.5 &\textbf{55.1} &66.9 &35.0 &\textbf{56.2} &33.5 & \textbf{41.0}& \textbf{54.3}&\textbf{49.1}\textcolor{blue}{\tiny{(+22.1)}}\\
% \hline
% \end{tabular}
% \end{table}

\begin{table}[!tp]\centering
\scriptsize
\captionsetup{skip=0pt, position=above} % Force the caption to be above the table
\caption{\textbf{Domain adaptation.} City\textrightarrow Foggy in mAP ($\%$), $\dagger$ borrowed from \cite{he2022cross}.}
\label{tab:uda-c2fc}
\begin{tabular}{l|@{\hspace{3pt}}l@{\hspace{2pt}}|cccccccc|l}
\hline
 &\textbf{Method}  &\textbf{prsn} &\textbf{rider} &\textbf{car} &\textbf{truck} &\textbf{bus} &\textbf{train} &\textbf{motor} 
&\textbf{bike} & \textbf{mAP} \\
\hline
\multirow{2}{*}{-}&F-RCNN$\dagger$ \cite{ren2015faster}& 36.9 & 36.1 & 44.5.6& 21.7& 32.3&9.2 & 21.5& 32.4&28.3 \textcolor{red}{\tiny{(-20.8)}} \\
&R-CLIP \cite{zhong2022regionclip} &46.5 &51.8 &57.6 &27.3 &45.1 & 19.7& 34.8& 50.2 &\textbf{41.6} \textcolor{red}{\tiny{(-7.5)}} \\
\hline
 \multirow{9}{*}{DA}&SW-DA \cite{saito2019strong} \tiny(CVPR'19) &31.8 & 44.3&48.9 &21.0 &43.8 &28.0&28.9 &35.8& 35.3\\
% &DA-Faster$\dagger$ \cite{chen2018domain}\tiny(CVPR'18) &29.2 & 40.4&43.4 &19.7 &38.3 &28.5&23.7 &32.7& 32.0\\
 &D\&Match$\dagger$ \cite{kim2019diversify} \tiny(CVPR'19)  &31.8 &40.5 &51.0 &20.9  &41.8 &34.3 &26.6 &32.4 & 34.9\\
 &SC-DA$\dagger$ \cite{zhu2019adapting} \tiny(CVPR'19)&33.8&42.1&52.1&26.8&42.5&26.5&29.2&34.4&35.9\\
 &MTOR \cite{cai2019exploring} \tiny(CVPR'19)  &30.6 &41.4 &44.0 &21.9  &38.6 &40.6 &28.3 &35.6 & 35.1\\
 &AFAN$\dagger$ \cite{wang2021afan} \tiny{(TIP'21)}&42.5&44.6&57.0&26.4&48.0&28.3&33.2&37.1&39.6\\
&GPA$\dagger$ \cite{xu2020cross} \tiny(CVPR'20)  & 32.9&46.7 &54.1 &24.7 &45.7 &41.1 &32.4 &38.7 & 39.5\\ 
 &ViSGA$\dagger$ \cite{Rezaeianaran_2021_ICCV} \tiny{(ICCV'21)}&38.8&45.9&57.2&29.9&50.2&\textbf{51.9}&31.9&40.9&43.3\\
 &SFA$\dagger$ \cite{wang2021exploring} \tiny{(acmmm'21)}&46.5&48.6&62.6&25.1&46.2&29.4&28.3&44.0&41.3\\
&DSS$\dagger $\cite{wang2021domain} \tiny{(CVPR'21)}&\textbf{50.9}&\textbf{57.6}&61.1&\textbf{35.4}&50.9&36.6&38.4&51.1&47.8\\
 % &MKT$\dagger$ \cite{csaba2021multilevel}&43.5&52.0&63.2&34.7&52.7&45.8&37.1&49.4&47.3\\
 
 % &ICR-CCR \cite{xu2020exploring} \tiny(CVPR'20) &32.9 &43.8 &49.2 &27.2 &45.1 &36.4 &30.3 &34.6 & 37.4\\
 % &Coarse-to-Fine \cite{zheng2020cross} \tiny(CVPR'20)  & 34.0& 46.9& 52.1& 30.8& 43.2& 29.9& 34.7& 37.4& 38.6\\
 
 % &Center-Aware \cite{hsu2020every} \tiny(ECCV'20)  &41.5 &43.6 &57.1 &29.4 &44.9 &39.7 &29.0 &36.1 & 40.2\\ 
 % &CycConf \cite{wang2021robust}\tiny(ICCV'21)  &45.8 &51.0 &63.1 &26.8 &47.1 &23.6 & 30.6& 43.6&41.5 \\
 &TTD+FPN$\dagger$ \cite{he2022cross} \tiny(CVPR'22) & 50.7 & 53.7 & \textbf{68.2} & 35.1 & 53.0 & 45.1 & 38.9 &49.1 & \textbf{49.2}\\
 &IRG\tablefootnote{Source-free domain adaptation} \cite{vs2022instance} \tiny(CVPR'23)  & 37.4& 45.2& 51.9& 24.4& 39.6& 25.2& 31.5 &41.6 &  37.1\\
 \hline
 \multirow{2}{*}{DG}&DIDN \cite{lin2021domain} \tiny(ICCV'21)  &38.3 &44.4 &51.8 &28.7 &53.3 &34.7 &32.4 & 40.4&40.5 \textcolor{red}{\tiny{(-8.6)}} \\
&\textbf{Ours}  &50.5 &55.1 &66.9 &35.0 &\textbf{56.2} &33.5 & \textbf{41.0}& \textbf{54.3}&\textbf{49.1} \\
% \textcolor{blue}{\tiny{(+22.1)}}\\
\hline
\end{tabular}
\end{table}
\textbf{Extension to domain adaptation.} Our method can naturally extend to domain adaptation as it requires only one labeled source data. The labeled and unlabeled source domains serve as source and target domains, respectively. Table \ref{tab:uda-c2fc} presents the result of City to Foggy adaptation against baselines and sota DA methods, while real-to-artistic adaptation can be found in the supplement. As illustrated in Table \ref{tab:uda-c2fc}, our method improves Faster-RCNN and RegionCLIP by $20.8\%$ and $7.5\%$.
%, respectively. Additionally, 
It not only substantially outperforms DIDN (sota DGOD on this setting) by $8.6\%$ but also achieves comparable results to the existing DA works. It slightly underperformed compared to TTD by only $0.1\%$, but in contrast to DA methods, our method is not designed to adapt to a particular domain.

\subsection{Ablation Studies}
\label{sec:ablation}
\begin{table*}[!tp]
\scriptsize
\captionsetup{skip=0pt, position=above} 
\caption{\textbf{Ablation studies}. \textit{Domain Generalization} (VOC,Clipart $\rightarrow$ Watercolor,Comic), \textit{Domain Adaptation} (VOC $\rightarrow$ Clipart). Results in mAP (\%).}
\label{tab:ablation_all}
\begin{subtable}[b]{0.44\linewidth}
\scriptsize
\centering
    \begin{tabular}{|l@{\hspace{2pt}}|c@{\hspace{3pt}}|@{\hspace{3pt}}c@{\hspace{3pt}}c@{\hspace{3pt}}|}
        \hline
        {\textbf{Method}} &
        {DA} &\multicolumn{2}{c|}{{DG}}\\
        \cline{2-4}
         &{Clipart} &{Watercolor} &{Comic} \\
        \hline
        F-RCNN  \cite{ren2015faster}  &24.1 \textcolor{red}{\tiny{(-16.3)}} &41.2 \textcolor{red}{\tiny{(-8.6)}} &17.9 \textcolor{red}{\tiny{(-28.0)}} \\
        R-CLIP \cite{zhong2022regionclip}  &32.3 \textcolor{red}{\tiny{(-8.1)}} &44.7 \textcolor{red}{\tiny{(-5.1)}} &34.2 \textcolor{red}{\tiny{(-11.7)}} \\
        \hline
        DVA  &\underline{36.6} \textcolor{red}{\tiny{(-3.8)}} &\underline{45.6} \textcolor{red}{\tiny{(-4.2)}} &\underline{38.1} \textcolor{red}{\tiny{(-7.8)}} \\
        Caption-PL &35.2 \textcolor{red}{\tiny{(-5.2)}} &45.0 \textcolor{red}{\tiny{(-4.8)}} &36.4 \textcolor{red}{\tiny{(-9.5)}} \\
        % Ours (w/o KD)  &\underline{38.9}\textcolor{red}{\tiny{(-1.4)}}& \underline{46.4}\textcolor{red}{\tiny{(-3.2)}}& 36.9\textcolor{red}{\tiny{(-9.0)}}\\
        % Ours (w/o KD)  &\underline{35.1}\textcolor{red}{\tiny{()}}& \underline{43.8}\textcolor{red}{\tiny{()}}& 
        % 35.9\textcolor{red}{\tiny{()}}\\ 
        Ours &\bfseries40.4 &\bfseries49.8 &\bfseries45.9 \\
        \hline
    \end{tabular}
    \caption{Lang. guided feature alignment ablation}
    \label{tab:ablation_a}
\end{subtable}
\hfill
\begin{subtable}[b]{0.55\linewidth}
\centering
    \begin{tabular}{|@{\hspace{2pt}}l@{\hspace{3pt}}l@{\hspace{3pt}}l@{\hspace{3pt}}l@{\hspace{3pt}}|@{\hspace{3pt}}c@{\hspace{3pt}}|c@{\hspace{3pt}}c@{\hspace{3pt}}|}
        \hline
        &&&  &DA & \multicolumn{2}{c|}{DG}\\
        R-CLIP init & $\mathcal{L}_{img-cont}$ &  $\mathcal{L}_{inst-cont}$ & $\mathcal{L}_{dist}$ & Clipart & Watercolor&Comic \\
        \hline
        &&&  &24.1&41.2&17.9\\
        $\checkmark$&&&& 32.3&44.7&34.2\\
        \hline
        $\checkmark$& $\checkmark$&&& 32.3&41.7&35.1 \\
        $\checkmark$& &$\checkmark$& & 34.6&45.0&35.4 \\
        $\checkmark$& $\checkmark$&$\checkmark$&&35.1&44.2&35.7 \\
        $\checkmark$& $\checkmark$&$\checkmark$ &$\checkmark$& \textbf{40.4}&\textbf{49.8}&\textbf{45.9} \\
\hline
\end{tabular}
        \caption{Effectiveness of each component}
        \label{tab:ablation_b}
    \end{subtable}
    \vspace{-10.0pt}
\end{table*}

We conduct an extensive ablation study by examining four aspects of our method: (i) the impact of vision-language pre-training (Sec.~\ref{sec:supervised}), (ii) the effectiveness of language space alignment compared to visual-space alignment (Sec.~\ref{sec:CDDMSL}), (iii) the benefit of feature-space objective compared to token-space objective, and (iv) the contribution of knowledge distillation regularization (Sec.~\ref{sec:KD}) in Table \ref{tab:ablation_a}. Table \ref{tab:ablation_b} exhibits the effectiveness of each component of the proposed method. 
%All experiments are conducted on the \textit{VOC,Clipart$\rightarrow$Comic,Watercolor} setting.

\textbf{Language space vs. visual space alignment.}
    To better understand the effectiveness of enforcing domain-invariant learning through language space, we compare with the Direct Visual Alignment  baseline (third row of Table \ref{tab:ablation_a}) under an identical setting. In all settings, ours (last row) substantially exceeds DVA in both DA and DG tasks. %Moreover, ours without KD (fifth row) also performs better than DG in two out of three domains. This shows the superior impact of enforcing feature alignment through the language space. 

\textbf{Feature-space vs. token-space.} Comparing Caption-PL (row 4) with our approach in Table \ref{tab:ablation_a} shows the superiority of enforcing consistency in the embedding space rather than token space. Ours achieves significant improvement over Caption-PL by $5.2\%$, $4.8\%$, and $9.5\%$. Token space approaches may degrade the model's performance by focusing on unnecessary tokens without meaningful information. 
%Additionally, token generation is non-differentiable, making it challenging to deploy such methods in practice.

% In all settings, Comparing Caption-PL (row 4), token-space pseudo labeling baseline (see baselines), with Ours w/o KD and with KD ( row 7 and row 8) in Table \ref{tab:ablation_a} shows the superiority of enforcing the consistency in the embedding space rather than tokens space. Particularly, Ours + KD (last row) achieves $4.9\%$, $4.0\%$, and $11.0\%$ improvement compared to Caption-PL. This can be due to the fact that not all tokens contain meaningful information. Therefore, the model's performance may degrade by focusing on producing consistent predictions for unnecessary tokens rather. On the other hand, feature space helps the model to focus on the overall semantics of the image. Moreover, another downside of token space is that token generation is non-differentiable, which makes deploying such methods difficult in practice.

\textbf{Effectiveness of each component.} Table \ref{tab:ablation_b} shows that instance-level is slightly more effective than image-level, while multi-scale (fifth row) can slightly improve the result. This indicates the importance of mitigating bias and distribution shifts at both levels, especially instance-level in object detection. Finally, adding a knowledge distillation regularizer results in the best performance (compare the last two rows). This supports our argument that our knowledge regularization helps the model avoid trivial solutions and focus on producing semantically consistent descriptions.















% \begin{table}[!tp]\centering
% \captionsetup{skip=0pt, position=above} % Force the caption to be above the table
% \caption {Ablation Study- \textbf{Domain Generalization} (VOC, Clipart $\rightarrow$ Watercolor, Comic) and \textbf{Domain Adaptation }(VOC $\rightarrow$ Clipart). Results in mAP(\%)} 
% \label{tab:ablation}  
% \scriptsize
% \begin{tabular}{l|c|c|cc}
% % \bottomrule
% \toprule
% {\textbf{Method}} & \textbf{Source}&
% \textbf{DA} &\multicolumn{2}{c}{\textbf{DG}}\\
% \cline{2-5}
% &\textbf{VOC} &\textbf{Clipart} &\textbf{Watercolor} &\textbf{Comic} \\
% \hline
% Faster-RCNN  \cite{ren2015faster} &80.3 &24.1\textcolor{red}{\tiny{16.2}} &41.2\textcolor{red}{\tiny{0}} &17.0\textcolor{red}{\tiny{0}} \\
% RegionCLIP \cite{zhong2022regionclip}  &77.1 &33.8\textcolor{red}{\tiny{6.5}} &44.7\textcolor{red}{\tiny{4.9}} &34.2\textcolor{red}{\tiny{11.7}} \\
% \hline
% Direct Visual Alignment &75.8 &37.5\textcolor{red}{\tiny{2.8}} &45.6\textcolor{red}{\tiny{4.0}} &38.1\textcolor{red}{\tiny{7.8}} \\
% Caption-PL  &77.2 &35.4\textcolor{red}{\tiny{4.9}} &45.6\textcolor{red}{\tiny{4.0}} &34.9\textcolor{red}{\tiny{11.0}} \\
% % @non contrastive loss & & & & \\
% \hline
% Ours(only image-level, w/o KD) & 77.3& 33.0\textcolor{red}{\tiny{7.3}} & 41.7\textcolor{red}{\tiny{7.9}}& 35.1\textcolor{red}{\tiny{10.8}} \\
% Ours(only region-level, w/o KD) &77.5 &34.6\textcolor{red}{\tiny{5.7}} & 44.8\textcolor{red}{\tiny{4.8}}& 35.4\textcolor{red}{\tiny{10.5}}\\
% Ours (multi-scale, w/o KD) &79.5 &38.9\textcolor{red}{\tiny{1.4}}& 46.4 \textcolor{red}{\tiny{3.2}}& 36.9\textcolor{red}{\tiny{9}}\\
% Ours (multi-scale + KD) &76.6 &\bfseries40.3 &\bfseries49.6 &\bfseries45.9 \\
% \hline
% \end{tabular}
% \end{table}
